Identifying human values from goal models: An industrial case study

Human values are principles that guide human actions and behaviour in personal and social life. Ignoring human values during requirements engineering introduces a negative impact on software uptake and continued use. Embedding human values into software is admittedly challenging; however, early elicitation of stakeholder values increases the chances of their inclusion into the developed system. Using Pharaon, a research and innovation project of the European Union's Horizon 2020 program, as a case study we analysed stakeholder requirements expressed as motivational goal models consisting of functional, quality, and emotional goals in three large-scale trial applications of the project. We were able to elicit 9 of 10 human values according to the theory of human values by Schwartz from the motivational goal models that represent the requirements for the three applications. Our findings highlight the dominant trend of stakeholder values being embedded in emotional goals and show that almost 45% of the identified values belong to the value categories of Security and Self-direction. Our research extends prior work in emotional goal modelling in requirements engineering by linking emotional goals to various stakeholder roles and identifying their values based on the Schwartz theory of human values

==> Tables/EmotionCount.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
Emotional Goals & Italy                             & Slovenia                          & Netherlands & \# \\ \hline
Informed       & 2                                 & 3                                 & {\color[HTML]{FF0000} \textbf{0}}   & 5  \\ \hline
Empowered      & 2                                 & 2                                 & 1                                   & 5  \\ \hline
In touch        & 2                                 & 1                                 & {\color[HTML]{FF0000} \textbf{0}}   & 3  \\ \hline
Involved       & 2                                 & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}}   & 2  \\ \hline
Stress free  & 1 & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1 \\ \hline
Reassured      & 1                                 & 1                                 & 1                                   & 3  \\ \hline
Safe           & 1                                 & 2                                 & 2                                   & 5  \\ \hline
Active         & 1                                 & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}}   & 1  \\ \hline
Motivated      & 2                                 & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}}   & 2  \\ \hline
Interested     & 1                                 & 1                                 & {\color[HTML]{FF0000} \textbf{0}}   & 2  \\ \hline
Incentivised & 1 & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1 \\ \hline
Aware          & 1                                 & 2                                 & {\color[HTML]{FF0000} \textbf{0}}   & 3  \\ \hline
Cared for      & {\color[HTML]{FF0000} \textbf{0}} & 2                                 & {\color[HTML]{FF0000} \textbf{0}}   & 2  \\ \hline
Included       & {\color[HTML]{FF0000} \textbf{0}} & 1                                 & {\color[HTML]{FF0000} \textbf{0}}   & 1  \\ \hline
Engaged        & {\color[HTML]{FF0000} \textbf{0}} & 1                                 & {\color[HTML]{FF0000} \textbf{0}}   & 1  \\ \hline
Confident      & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Private        & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Together       & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Supported      & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 2                                   & 2  \\ \hline
Heard          & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Belonging      & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Enjoyed        & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Nostalgic      & {\color[HTML]{FF0000} \textbf{0}} & {\color[HTML]{FF0000} \textbf{0}} & 1                                   & 1  \\ \hline
Total          & 17                                & 16                                & 13                                  & 46 \\ \hline
\end{tabular}%
}
\caption{Frequencies of emotions in the project}
\label{tab:my-table}
\end{table}

==> Tables/HumanvalueItemsvsEmotion.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l |l |l |l |}
\hline
\textbf{Value Category}                                  & \textbf{Value Item}                 & \textbf{\#} & \textbf{Emotional Goal}                           \\ \hline
  & Freedom                             & 4              & Empowered, In touch                               \\ \cline{2-4} 
   & Independence                        & 6              & Involved, Stress free, Informed                   \\ \cline{2-4} 
   & Privacy                             & 4              & Stress free, Aware, Empowered, Private            \\ \cline{2-4} 
 & Choosing own goals                  & 3              & Empowered, Involved                               \\ \cline{2-4} 
   & Curiosity                           & 2              & Interested                                        \\ \cline{2-4} 
\multirow{-6}{*}{Self-direction} & Self-respect                        & 5              & Informed, Empowered                              \\ \hline
                                & Excitement in life                   & 6              & Together, Involved, In touch, Interested, Engaged \\ \cline{2-4} 
\multirow{-2}{*}{Stimulation}    & A varied life                       & 2              & Active, Interested                                \\ \hline
&
  Pleasure &
  6 &
  \begin{tabular}[c]{@{}l@{}}Incentivised, Nostalgic, Stress free, Enjoyed, \\ Motivated, Cared for\end{tabular} \\ \cline{2-4} 
\multirow{-2}{*}{Hedonism} &
  Enjoying life &
  5 &
  Nostalgic, Stress free, Enjoyed, Motivated, Incentivised \\ \hline
                                & Ambitious                           & 1              & Motivated                                         \\ \cline{2-4} 
                                & Influential                         & 1              & Aware                                             \\ \cline{2-4} 
                                & Capable                             & 6              & Aware, Empowered, Confident                      \\ \cline{2-4} 
\multirow{-4}{*}{Achievement}    & Successful                          & 1              & Confident                                         \\ \hline
                                & Authority                           & 4              & Aware, Reassured, Informed                        \\ \cline{2-4} 
                                & Preserving my public image          & 1              & Empowered                                         \\ \cline{2-4} 
                                & Recognition                         & 2              & Reassured,  Empowered                             \\ \cline{2-4} 
\multirow{-4}{*}{Power}          & {Social power} & 1              & Informed                                          \\ \hline
&
  Sense of belonging &
  11 &
  \begin{tabular}[c]{@{}l@{}}Informed, In touch, Supported, Cared for\\ Belonging, Included, Involved\end{tabular} \\ \cline{2-4} 
                                & Social order                        & 5              & Safe, Informed, Private                           \\ \cline{2-4} 
                                & Healthy                             & 8              & Informed, Safe, Cared for, Reassured              \\ \hline
\multirow{-5}{*}{Security} &
  {\color[HTML]{000000} Honoring of parents and elders} & 4 &  Aware, Informed, Reassured \\ \cline{2-4}
  \multirow{-2}{*}{Conformity} &
                                 Politeness                             & 4              & Aware, Informed, Reassured                    \\ \hline

                                  
                                 &Helpful                             & 4              & Informed, Reassured, Together                     \\ \cline{2-4} 
                                & Responsible                         & 3              & Reassured, Together                               \\ \cline{2-4} 


\multirow{-3}{*}{Benevolence} &
  True friendship &
  6 &
  In touch, Together, Involved, Belonging \\ \hline
                                & Equality                            & 1              & Included                                          \\ \cline{2-4} 
\multirow{-2}{*}{Universalism}   & Wisdom                              & 1              & Nostalgic                                         \\ \hline
\end{tabular}%
}
\caption{The presence of value items with their respective categories}
\label{tab:humanvalueitemsandCategoriesvsemotion}
\end{table}

==> Tables/slovenia_humanvalue_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
{\color[HTML]{000000} \textbf{Functional Goal}} &
  {\color[HTML]{000000} \textbf{Role}} &
  {\color[HTML]{000000} \textbf{Emotional Goals}} &
  {\color[HTML]{000000} \textbf{Human Values}} \\ \hline
{\color[HTML]{000000} Improve well-being} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Safe} &
  {\color[HTML]{000000} Security : Social order, Healthy} \\ \hline
{\color[HTML]{000000} Improve well-being} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Empowered} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Achievement : Capable, \\ Self-direction : Self-respect\end{tabular}} \\ \hline
{\color[HTML]{000000} Improve well-being} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Informed} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Security : Healthy, Sense of belonging\\ Self-direction : Independence, Self-respect\end{tabular}} \\ \hline
{\color[HTML]{000000} Improve well-being} &
  {\color[HTML]{000000} CG} &
  {\color[HTML]{000000} Informed} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Conformity : Politeness, Honoring parents and elders\\ Power :  Authority\end{tabular}} \\ \hline
{\color[HTML]{000000} Get informed about monitoring} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Aware} &
  {\color[HTML]{000000} Self-direction : Privacy, Independence} \\ \hline
{\color[HTML]{000000} Discuss results} &
  {\color[HTML]{000000} CG} &
  {\color[HTML]{000000} Aware} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Conformity : Politeness, Honoring parents and elders\\ Power :  Authority\end{tabular}} \\ \hline
{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Discuss results\\ Trigger alarm\end{tabular}} &
  {\color[HTML]{000000} CG} &
  {\color[HTML]{000000} Reassured} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Conformity : Politeness, Honoring parents and elders\\ Benevolence : Responsible, Helpful\end{tabular}} \\ \hline
{\color[HTML]{000000} Discuss results} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Cared for} &
  {\color[HTML]{000000} Security : Healthy, Sense of belonging} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Safe} &
  {\color[HTML]{000000} Security : Social order, Healthy} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Informed} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Security : Healthy, Sense of  belonging\\ Self-direction : Independence, Self-respect\end{tabular}} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Empowered} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Achievement: Capable, \\ Self-direction : Freedom\end{tabular}} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Cared for} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Security : Sense of belonging \\ Hedonism : Pleasure\end{tabular}} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Included} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Universalism : Equality \\ Security : Sense of belonging\end{tabular}} \\ \hline
{\color[HTML]{000000} Participate in the community} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Engaged} &
  {\color[HTML]{000000} Stimulation : Excitement in Life} \\ \hline
{\color[HTML]{000000} Communicate with others} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} In touch} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Benevolence : True friendship \\ Self-direction : Freedom \\ Security : Sense of belonging\end{tabular}} \\ \hline
{\color[HTML]{000000} Participate in events} &
  {\color[HTML]{000000} OA} &
  {\color[HTML]{000000} Interested} &
  {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Stimulation : Excitement in life, Varied life\\ Self-direction : Curiosity\end{tabular}} \\ \hline
\end{tabular}%
}
\floatfoot{\quad\textsuperscript{\thempfootnote} OA= Older Adults, CG= Caregiver}
\caption{Mapping of goal models of the Slovenian pilot to the human values by Schwartz}

\label{tab:slovenia_humanvalue}
\end{table}
